Symmetrized Robust Procrustes: Constant-Factor Approximation and Exact Recovery

The classical $\textit{Procrustes}$ problem is to find a rigid motion (orthogonal transformation and translation) that best aligns two given point-sets in the least-squares sense. The $\textit{Robust Procrustes}$ problem is an important variant, in which a power-1 objective is used instead of least squares to improve robustness to outliers. While the optimal solution of the least-squares problem can be easily computed in closed form, dating back to Sch\"onemann (1966), no such solution is known for the power-1 problem. In this paper we propose a novel convex relaxation for the Robust Procrustes problem. Our relaxation enjoys several theoretical and practical advantages: Theoretically, we prove that our method provides a $\sqrt{2}$-factor approximation to the Robust Procrustes problem, and that, under appropriate assumptions, it exactly recovers the true rigid motion from point correspondences contaminated by outliers. In practice, we find in numerical experiments on both synthetic and real robust Procrustes problems, that our method performs similarly to the standard Iteratively Reweighted Least Squares (IRLS). However the convexity of our algorithm allows incorporating additional convex penalties, which are not readily amenable to IRLS. This turns out to be a substantial advantage, leading to improved results in high-dimensional problems, including non-rigid shape alignment and semi-supervised interlingual word translation.

==> content/rigid_motion.tex <==
\section{Rigid motion recovery}

We now consider a more general problem, whereby the inlier point correspondences are created by a rigid motion rather than merely by an orthogonal matrix. Suppose that we are given $P = \brc{p_1,\ldots,p_n}$ and $Q = \brc{q_1,\ldots,q_n}$, and $\p[i] = R_0 \p[i] - t_0$ for $i \in \I$, where $R_0$ is a $d \times d$ orthogonal matrix as before, and $t_0 \in \R[d]$ is a translation vector. Our proposed approach is to iterate over the indices $i$, each time translating $\p[i]$ and $\p[i]$ to the origin and solving the Orthogonal Procrustes problem over the translated sets. This approach is summarized in \cref{alg_rigid}.

\begin{algorithm}
    \caption{Seek a rigid motion that solves the robust procrustes problem}\label{alg_rigid}
    %\floatfoot{This is a float foot}
    %\algDescription{Here we can say a few words about the algorithm.}
    \begin{algorithmic}[1]
    \Input $P = \brc{p_1,\ldots,p_n}$, $Q = \brc{q_1,\ldots,q_n}$
    \Output Orthogonal matrix $U \in \R[d\times d]$ and translation vector $t \in \R[d]$
    \For{$i=1,\ldots,n$}
        \State Set $\tilde{P} \leftarrow \brc{p_1-\p[i],p_2-\p[i],\ldots,p_n-\p[i]}$ and $\tilde{Q} \leftarrow \brc{q_1-\p[i],q_2-\p[i],\ldots,q_n-\p[i]}$
        \State Let $A_i$ be a global minimizer of \cref{pr:relax_orth} with $\tilde{P}$, $\tilde{Q}$
        \State Set $R_i \leftarrow \Pi\br{A_i}$
        \State Set $t_i \leftarrow R_i \p[i] - \p[i]$
    \EndFor
    \State\Return $\br{U_i,t_i}$ for $i$ that yield the smallest objecive
    \end{algorithmic}
    \end{algorithm}
    

==> content/snippets.tex <==
From intro:
A well-known example of this approach is in the field of sparse regression analysis \cite{tibshirani1996regression} and compressed sensing \cite{donoho2006compressed,candes2006stable}, where an $\ell_2$ Tikhonov regularizer is replaced by the $\ell_1$ Lasso, which leads to improved results in tasks such as sparse signal recovery. In light of these results, one would expect this power-1 formulation to be less sensitive to erroneously matched pairs of point $\p[i]$ and $\q[i]$ compared to the least-squares objective of \cref{pr:procrustes_rigid}.


Notation and preliminaries:
$I_d$ is the $d \times d$ identity matrix and $\zeromat$ is the zero matrix. $SO\br{d}$ denotes the set of rotation matrices $\set{R \in O\br{d}}{\det\br{R}=1}$. For $A \in \R[d \times d]$, $\diag{A}$ is the vector $v \in \R[d]$ such that $v_k=a_{kk}$ for $k \in \brs{d}$. Conversely, $\diag{v}$ for $v \in \R[d]$ is the $d \times d$ diagonal matrix $A$ such that $a_{kk} = v_k$ for $k \in \brs{d}$. For a positive integer $n$, $\brs{n}$ denotes the set $\brc{1,\ldots,n}$. $O\br{d}$ denotes the set of $d \times d$ orthogonal matrices $\set{A \in \R[d\times d]}{A^T A = I_d}$


\begin{enumerate}
	\item We provide $\sqrt{2}$-factor approximation algorithm for the robust Procrustes problem, which runs in  by a polynomial-time algorithm. 
	\item We prove that under certain assumptions, recovery problems with outliers but without noise can be solved exactly in polynomial time by our algorithm.
	\item Our \SRP algorithms provide lower bounds that can be used to evaluate other methods, and for branch and bound algorithms. 
	\item For robust Procrustes problems with additional convex energy terms, we demonstrate empirically that our \SRP method is superior to existing alternatives.  
\end{enumerate}

Non-symmetrized relaxation:
\begin{equation}\label{pr:nonsym_rigid}
   \min_{A \in \R[d\times d], t \in \R[d]} \sum_{i=1}^n \norm{A \p[i]+t-\q[i]}
\end{equation}

==> content/text/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% 	justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
% 	\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
% 	\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% 	\item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}
	
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? 
		\answerYes{Yes. Our claims about our paper's contributions made in the abstract and introduction are discussed in detail in the theory section \ref{sec_theory} and demonstrated empirically in \cref{sec_numerical_experiments}.}
		%
		\item Did you describe the limitations of your work?
		\answerYes{In the introduction we discuss settings in which our method does not achieve superior performance over the IRLS method, and visualize them in \cref{sec_numerical_experiments}, alongside other settings where our method ourperforms the competition; see, for example, \cref{fig_recovery_R}.}
		%
		\item Did you discuss any potential negative societal impacts of your work?
		\answerNo{We are not aware of any potential negative societal impacts related to the robust Procrustes problem.}
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes{}
	\end{enumerate}
	
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerYes{All the theoretical claims in this paper are clearly stated, including their full set of assumptions.}
		\item Did you include complete proofs of all theoretical results?
		\answerYes{The complete proofs of all theoretical results in this paper appear in the appendix.}
	\end{enumerate}
	
	
	\item If you ran experiments...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerYes{All experimental results presented in this paper are fully reproducible. We intend to upload the code required to reproducte our results by the submission deadline for supplementary materials.}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerYes{Our experimental settings are described in detail in \cref{app_technical_details}.}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerNo{For most experiments we did not include error bars. In all of our experiments, except for the NLP \cref{table_nlp1}, we took the average results over 200 independent instances, which should be enough to exclude the possibility of large apparent performance gaps that are due to statistical error. In the NLP results, where we took averages over 10 instances due to time constraints, we report $\SI{95}{\percent}$ confidence intervals.}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerYes{The running times of our method and full details about hardware used are included in the appendix.}
	\end{enumerate}
	
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerYes{We cited the creators of all the code and data used in our experiments.}
		\item Did you mention the license of the assets?
		\answerNo{We have not yet been able to find the licenses of all assets used in our paper. We intend to look for them.}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerYes{We incude code in the supplementary material.}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerNA{All data used in our work was published by its creators.}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerNA{We are not using personally identifiable information or offensive content.}
	\end{enumerate}
	
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{We did not use crowdsourcing or conducted research with human subjects.}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{See above.}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
		\answerNA{See above.}
	\end{enumerate}
	
	
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> content/text/subsection_previous_works.tex <==
\subsection{Previous works}\label{subsec_previous_works}
-TBD-

==> packages/set_figures.tex <==
\newcommand{\figDescriptionTextSize}{\footnotesize}


==> packages/set_graphics.tex <==
\usepackage{graphicx}
%
\usepackage{epstopdf}
\epstopdfDeclareGraphicsRule{.eps}{pdf}{.pdf}{%
  epstopdf --gsopt=-dCompatibilityLevel=1.5 "--outfile=\OutputFile" "#1" }
% 
\graphicspath{{eps/}}  

